The degrees of freedom of the Group Lasso for a General Design

In this paper, we are concerned with regression problems where covariates can be grouped in nonoverlapping blocks, and where only a few of them are assumed to be active. In such a situation, the group Lasso is an at- tractive method for variable selection since it promotes sparsity of the groups. We study the sensitivity of any group Lasso solution to the observations and provide its precise local parameterization. When the noise is Gaussian, this allows us to derive an unbiased estimator of the degrees of freedom of the group Lasso. This result holds true for any fixed design, no matter whether it is under- or overdetermined. With these results at hand, various model selec- tion criteria, such as the Stein Unbiased Risk Estimator (SURE), are readily available which can provide an objectively guided choice of the optimal group Lasso fit.

==> sections/gsure_rel.tex <==
\section{Degrees of freedom and Risk Estimation}
\label{sec:dof}

%Note that even if \lasso admits several solutions, all of them share the same image under $\XX$.
%Hence, we define without ambiguity $\widehat{\mu}(y) = \XX \xsoly(y)$ where $\xsoly(y)$ is any solution of \lasso. 
As remarked earlier and stated formally in Lemma~\ref{lem:same-image}, all solutions of the Lasso share the same image under $\XX$, hence allowing us to denote the prediction $\widehat{\mu}(y)$ without ambiguity as a single-valued mapping. The next theorem provides a closed-form expression of the local variations of $\widehat{\mu}(y)$ with respect to the observation $y$. In turn, this will yield an unbiased estimator of the degrees of freedom and of the prediction risk of the group Lasso.
\begin{thm}\label{thm-div}
  Let $\lambda > 0$.
  For all $y \not\in \Hh$, there exists a solution $\xsoly(y)$ of \lasso with \bsup $I = \bs(\xsoly(y))$ such that $({\rm\bf{A}}(\xsoly(y)))$ is fulfilled. Moreover, 
  The mapping $y \mapsto \widehat{\mu}(y)=X\xsoly(y)$ is $\Cc^1(\RR^n \setminus \Hh)$ and,
  \begin{equation}\label{eq:diverg}
    \diverg(\widehat{\mu}(y)) = \tr (\XX_I d(y,\lambda)) ~.
  \end{equation}
\end{thm}


\begin{thm}\label{thm-dofsure}
Let $\lambda > 0$. Assume $y = \XX \xx_0 + \epsilon$ where $\epsilon \sim \Nn(0,\sigma^2 \Id_n)$. The set $\Hh$ has Lebesgue measure zero, and therefore \eqref{eq:diverg} is an unbiased estimate of the DOF of the group Lasso. Moreover, an unbiased estimator of the prediction risk $\EE_\epsilon \norm{\widehat{\mu}(y) - \mu_0}^2$ is given by the $\SURE$ formula
\begin{align}
\label{eq:sure}
    \SURE(\xsoly) = &
    \norm{y - \widehat{\mu}(y)}^2
    - n \sigma^2
    + 2 \sigma^2 \tr (\XX_I d(y,\lambda))~.
\end{align}
\end{thm}

%This theorem shows that $\widehat{\DOF} = \XX_I d(y)$ is an unbiased estimate of the degrees of freedom.
% We can now give a closed-form expression for the Stein Unbiased Risk Estimator.
%   Let $\lambda > 0$.
%   Assume $y = \XX \xx_0 + \epsilon$ where $\epsilon \sim \Nn(0,\sigma^2 \Id_n)$.
%   Let $I = \bs(\xsoly(y))$, then the quantity
%   \begin{align*}
%     \SURE(\xsoly) = &
%     \norm{y - \widehat{\mu}(y)}^2
%     - n \sigma^2
%     + 2 \sigma^2 \tr (\XX_I d(y,\lambda))~,
%   \end{align*}
%   is an unbiased estimator of the prediction risk
%   $\EE_\epsilon \pa{ \normd{ \mu_0 - \widehat{\mu}(y)}^2 }$.

Although not given here explicitly, Theorem~\ref{thm-dofsure} can be straightforwardly extended to
unbiasedly of measures of the risk, including the {\it projection} risk, or the {\it estimation}
risk (in the full rank case) through the Generalized Stein Unbiased Risk Estimator as proposed in \citep{vaiter-local-behavior}.\\

An immediate corollary of Theorem~\ref{thm-dofsure} is obtained when $\XX$ is orthogonal, and without loss of generality $\XX=\Id_n$, i.e. the block soft thresholding estimator. In particular, we recover the expression found by \citep{yuan2006model}.
\begin{cor}\label{cor-particular}
  If $\XX = \Id_n$, then
  \begin{equation*}
    \widehat{\DOF} = \abs{J} - \lambda \sum_{b \in J} \dfrac{\abs{b} - 1}{\norm{y_b}}
  \end{equation*}
  where $J = \bigcup \enscond{b \in \Bb}{\norm{y_b} > \lambda}$.
  Moreover, the $\SURE$ is given by
  \begin{align*}
    \SURE(\xsoly) = &
    -n \sigma^2
    +
    (2 \sigma^2 + \lambda^2) \abs{J}
    + \sum_{b \notin J} \norm{y_b}^2
    - 2 \sigma^2 \lambda \sum_{b \in J} \dfrac{\abs{b} - 1}{\norm{y_b}} ~.
  \end{align*}
%  is an unbiased estimator of the estimation risk $\EE_\epsilon \pa{ \normd{ \xx_0 - \xsoly(y)}^2 }$.
\end{cor}

We finally assess the (relative) reliability of the SURE by computing the expected squared-error between $\SURE(\xsoly(y))$ and the true squared-error on $\xsoly(y)$
\eq{
\SE(\xsoly(y)) = \norm{\widehat{\mu}(y)-\mu_0}^2 ~.
}
\begin{prop}\label{prop:rel}
Under the assumptions of Theorem~\ref{thm-dofsure}, the relative realibility obeys
\eq{
\EE_w\left[\frac{\pa{\SURE(\xsoly(y))-\SE(\xsoly(y))}^2}{n^2\sigma^4}\right] \leq \frac{18+4\norm{X_I^\ins{T}X_I \bpa{ \XXX + \lambda \delta_{\xsoly(y)}  \circ P_{\xsoly(y)}  }^{-1}}^2}{n} + \frac{8\norm{\mu_0}^2}{n^2\sigma^2} ~.
}
It has the rate  $O(1/n)$ if $\norm{X_I^\ins{T}X_I\bpa{ \XXX + \lambda \delta_{\xsoly(y)}  \circ P_{\xsoly(y)}  }^{-1}}=O(1)$.
\end{prop}
%%% Local Variables: 
%%% TeX-master: "../l1l2-variations-dof.tex"
%%% End: 


==> sections/proofs-dof_rel.tex <==
\subsection{Proof of Theorem \ref{thm-div}} % (fold)
\label{sub:dof}

We define the set
\begin{equation}\label{eq:cnd}
   \cnd_{I} =
   \enscond{\xx_I\in \RR^{\abs{I}}}
   {\forall \alpha \in \RR^{\abs{I}}, \sum_{b \in I} \alpha_b \XX_b^{} \xx_b = 0 \Rightarrow \alpha = 0} .
\end{equation}
It is easy to see that $\xxs \in \cnd_I$ for $I$ the \bsup of $\xxs$ if and only if $({\rm\bf{A}}(\xxs))$.

\medskip

The following lemma proves that there exists a solution $\xxs$ of \lasso such that $({\rm\bf{A}}(\xxs))$ holds. A similar result with a different proof can be found in \citep{LiuZhang09}.
\begin{lem}
  There exists a solution $\xxs$ of \lasso such that $\xxs \in \cnd_I$ where $I = \bs(\xxs)$.
\end{lem}
\begin{proof}
  Let $\xx^0$ be a solution of \lasso and $I = \bs(\xx^0)$ such that $\xx_I^0 \not\in \cnd_I$.
  There exists $\mu \in \RR^{\abs{I}}$ such that
  \begin{equation}\label{eq:inde}
    \sum_{b \in I} \mu_b \XX_b \xx_b^0 = 0 .
  \end{equation}
  Consider now the family $t \mapsto \xx^t$ defined for every $t \in \RR$
  \begin{equation}
    \forall b \in I, \quad \xx_b^t = (1 + t \mu_b) \xx_b^0 \qandq \beta^t_{I^c} = 0 ~.
  \end{equation}
  Consider $t_0 = \min \enscond{\abs{t} \in \RR}{\exists b \in I \text{ such that } 1 + t \mu_b = 0} $.
  Remark that for all $t \in [0,t_0)$, $\xx^t$ is a solution of \lasso.
  Indeed, $I$ is the \bsup of $\xx^t$ and
  \begin{equation}
    \XX_I \xx_I^t = \XX_I \xx_I^{0} + t \underbrace{\sum_{b \in I} \mu_b \XX_b \xx_b^0}_{=0 \text{ using \eqref{eq:inde}} } = \XX_I \xx_I^{0} .
  \end{equation}
  Hence, 
  \begin{equation*}
    \XX_I^{\ins{T}}(y - \XX_I \xx_I^t) 
    = \XX_I^{\ins{T}}(y - \XX_I \xx_I^{0})
    = \lambda \no(\xx_I)
    = \lambda \no(\xx_I^t) ,
  \end{equation*}
  and
  \begin{equation*}
    \norm{\XX_b^{\ins{T}}(y - \XX_I \xx_I^t)} = \norm{\XX_b^{\ins{T}}(y - \XX_I \xx_I)} \leq \lambda .
  \end{equation*}
  Since the image of all solutions of \lasso are equal under $\XX$, one has
  \begin{equation*}
    \XX \xx^{t} = \XX \xx^{0}
    \qandq
    \normg{\xx^{t}} = \normg{\xx^0} .    
  \end{equation*}
  where $\normg{\cdot}$ is the $\lun-\ldeux$ norm. Consider now the vector $\xx^{t_0}$.
  By continuity of $\xx \mapsto \XX \xx$ and $\xx \mapsto \normg{\xx}$, one has
  \begin{equation*}
    \XX \xx^{t_0} = \XX \xx^{0}
    \qandq
    \normg{\xx^{t_0}} = \normg{\xx^0} .
  \end{equation*}
  Hence, $\xx^{t_0}$ has a \bsup $I_{t_0}$ strictly included in $I$ (in the sense that for all $b \in I_{t_0}$ one has $b \in I$) and is a solution of \lasso.
  Iterating this argument with $\xx^0 = \xx^{t_0}$ shows that there exists a solution $\xxs$ such that $\xxs \in \cnd_{\bs(\xxs)}$. This concludes the proof of the lemma.
  
\medskip
  
According to Theorem \ref{thm-local}, $y \mapsto \xsoly(y)$ is $\Cc^1(\RR^n \setminus \Hh)$. This property is preserved under the linear mapping $\XX$ which shows that $\widehat{\mu}$ is also $\Cc^1(\RR^n \setminus \Hh)$. Thus, taking the trace of the Jacobian $X_I d(y,\lambda)$ gives the divergence formula \eqref{eq:diverg} for any solution $\xsoly(y)$ such that $({\rm\bf{A}}(\xsoly(y)))$ holds.
\end{proof}

\subsection{Proof of Theorem \ref{thm-dofsure}} % (fold)
\label{sub:sure}
\begin{proof}
The next lemma shows that the transition spaces have zero measure.
\begin{lem}
  Let $\lambda > 0$.
  The transition space $\Hh$ is of zero measure with respect to the Lebesgue measure of $\RR^n$.
\end{lem}
\begin{proof}
We obtain this result by proving that all $\Hh_{I,b}$ are of zero measure for all $I$ and $b \not\in I$, and that the union is over a finite set.

We recall from \citep{coste2002intro} that any semialgebraic set $S \subseteq \RR^n$ can be decomposed in a disjoint union of $q$ semialgebraic subsets $C_i$ each diffeomorphic to $(0,1)^{d_i}$.
The dimension of $S$ is thus
\begin{equation*}
  d = \umax{i \in \{1,\dots,q\}} d_i \leq n.
\end{equation*}
The set $\Aa_{I,b}$ is an algebraic, hence a semialgebraic, set.
By the fundamental Tarski-Seidenberg principle, the canonical projection $\pi(\Aa_{I,b})$ is also semialgebraic.
The boundary $\bd(\pi(\Aa_{I,b}))$ is also semialgebraic with a strictly smaller dimension than $\pi(\Aa_{I,b})$
\begin{equation*}
  \dim \Hh_{I,b}
  =
  \dim \bd(\pi(\Aa_{I,b}))
  <
  \dim \pi(\Aa_{I,b})
  \leq
  n
\end{equation*}
whence we deduce that $\Hh$ is of zero measure with respect to the Lebesgue measure on $\RR^n$.
\end{proof}

As $\widehat{\mu}$ is uniformly Lipschitz over $\RR^n$, using similar arguments as in \citep{MeyerWoodroofe}, we get that $\widehat{\mu}$ is weakly differentiable with an essentially bounded gradient. Moreover, the divergence formula \eqref{eq:diverg} holds valid almost everywhere, except on the set $\Hh$ which is of Lebesgue measure zero. We conclude by invoking Stein's lemma \citep{stein1981estimation} to establish unbiasedness of the estimator $\widehat \DOF$ of the DOF.


% We now recall Stein's lemma whose proof can be found in \cite{stein1981estimation}.
% \begin{lem}[Stein's lemma] \label{lem:stein}
% Let $y = \mu_0 + \epsilon$ with $\epsilon \sim \Nn(0,\sigma^2\Id_n)$.
% Assume that $g : y \mapsto g(y)$ is weakly differentiable,
% then
% \begin{align*}
%   \EE_\epsilon \dotp{\epsilon}{g(y)}
%   =
%   \si^2 \EE_\epsilon \diverg(g(y)) ~.
% \end{align*}
% 
% \end{lem}

Plugging the DOF expression into that of the $\SURE$ \citep[Theorem~1]{stein1981estimation}, we get \eqref{eq:sure}.
%   Since $y \mapsto \widehat{\mu}(y)=\XX \xsoly(y)$ is weakly differentiable,
%   we can apply Lemma~\ref{lem:stein}. We get
%   \begin{align*}
%     \EE_\epsilon \dotp{\epsilon}{  \widehat{\mu}(y)}
%     =
%     \sigma^2 \EE_\epsilon \diverg(\widehat{\mu}(y))~.
%   \end{align*}
%   Using the decomposition $ y =  \mu_0 +  \epsilon$, we obtain
%   \begin{align*}
%     \EE_\epsilon\normd{ y -  \widehat{\mu}(y)}^2
%     &=
%     \EE_\epsilon\normd{ \mu_0 +  \epsilon}^2
%     - 2 \EE_\epsilon \dotp{ \mu_0 +  \epsilon}{ \widehat{\mu}(y)}
%     + \EE_\epsilon\normd{ \widehat{\mu}(y)}^2\\
%     &=
%     \EE_\epsilon\normd{ \mu_0}^2 + n \si^2
%     - 2 \EE_\epsilon \dotp{  \mu_0}{ \widehat{\mu}(y)}
%     - 2 \EE_\epsilon \dotp{\epsilon}{  \widehat{\mu}(y)} 
%     + \EE_\epsilon \normd{ \widehat{\mu}(y)}^2\\
%     &=
%   \EE_\epsilon\normd{  \mu_0 -  \widehat{\mu}(y)}^2
%   + n \si^2
%   - 2 \si^2 \EE_\epsilon \diverg(\widehat{\mu}(y)) ~.
% \end{align*}
\end{proof}


\subsection{Proof of Corollary \ref{cor-particular}} % (fold)
\label{sub:proof-cor}
When $\XX = \Id$,  the solution of \lasso is a block soft thresholding
\begin{equation}\label{eq:block-soft}
  \xsoly_b(y)] = 
  \begin{cases}
      0 & \text{if } \norm{y_b} \leq \lambda \\
      (1 - \frac{\lambda}{\norm{y_b}}) y_b & \text{otherwise}
    \end{cases} .
\end{equation}
For every $b \in J$, we differentiate \eqref{eq:block-soft} to get
\begin{equation*}
  \partial_y \xsoly_b(y):  \alpha \in \RR^{\abs{b}} \mapsto \alpha - \frac{\lambda}{\norm{y_b}} P_{y_b^\bot}(\alpha) .
\end{equation*}
Since $P_{y_b^\bot}(\alpha)$ is a projector on a subspace of dimension $\abs{b} - 1$, one has $\tr (P_{y_b^\bot}) = \abs{b} - 1$.

\subsection{Proof of Proposition~\ref{prop:rel}}
From \cite{}, ...

% section proof -cor(end)
% Local Variables: 
% TeX-master: "../l1l2-variations-dof.tex"
% End:

